cuTeSpMM: Accelerating Sparse-Dense Matrix Multiplication using GPU Tensor Cores

Many recent GPUs feature matrix multiplication engines (aka Tensor Core Units or TCUs) that perform small fixed-size matrix-matrix products at very high throughput. They have been used very effectively to speed up dense matrix-matrix multiplication libraries like Nvidia's cuBLAS, enabling significantly higher performance over use of the traditional scalar GPU cores. There also been recent interest in using these dense TCUs for the important sparse-dense matrix-matrix multiplication (SpMM) kernel via explicit zero-filling. However, an examination of the attainable performance of TC-GNN, the state-of-the-art TCU-enhanced SpMM implementation, indicates that for a substantial majority of the sparse matrices in the SuiteSparse collection, the achieved performance falls significantly short of the state-of-the-art SpMM kernels that only utilize scalar cores. In this paper, we therefore address the question: Can dense TCUs be effectively used to accelerate SpMM for a range of sparse matrices arising from multiple application domains, such as those found in the SuiteSparse matrix collection? We answer this question in the affirmative by developing a very efficient TCU-based GPU kernel - cuTeSpMM (cuda Tensor core SpMM) that achieves substantially higher performance over TC-GNN. We also develop a notion of the TCU-Synergy of a sparse-matrix, based on its non-zero structure and a modeled Operational Intensity. For sparse matrices with high TCU-synergy, cuTeSpMM outperforms state-of-the-art scalar-core SpMM implementations, while achieving only slightly lower performance on matrices with low TCU-Synergy.

==> sections/abstract-old.tex <==
Many recent GPUs feature matrix multiplication engines (aka Tensor Core Units or TCUs) that perform small fixed-size matrix-matrix products at very high throughput. They have been used very effectively to speed up dense matrix-matrix multiplication libraries like Nvidia's cuBLAS, enabling significantly higher performance over use of the traditional scalar GPU cores. Since the peak performance of these TCUs can be almost an order-of-magnitude higher than the scalar GPU cores, there has been recent interest in using dense TCUs for sparse-dense matrix-matrix multiplication (SpMM), via explicit zero-filling of some sparse-matrix elements and thereby using the dense matrix-matrix multiplication instructions of the TCU. The Nvidia cuSparse library now also offers an SpMM implementation using TCUs for sparse matrices in a blocked-ELL format. Another TCU implementation of SpMM within a GNN implementation (TC-GNN) has reported high performance on some sparse matrices. However, the achieved performance of these existing TCU-based SpMM implementations is much lower than state-of-the-art SpMM using scalar cores for a significant fraction of the sparse matrices from the SuiteSparse collection. In this paper we take a systematic approach to analyze the characteristics of the pattern of non-zero elements in sparse matrices that may be conducive to achieving higher performance via a TCU-based SpMM implementation over one based on scalar cores, i.e., have {\em TCU-synergy}. An analysis of the sparse matrices in the SuiteSparse collection suggests that a surprisingly large number of them have TCU-Synergy, compared to the low fraction exhibiting good performance with existing TCU-based SpMM implementations. Motivated by these observations, we develop a very efficient TCU-based GPU kernel - cuTeSpMM (cuda Tensor core SpMM) that achieves substantially higher performance over existing TCU-based SpMM kernels across all matrices classes. For sparse matrices with TCU-synergy, as well as cuTeSpMM outperforms state-of-the-art scalar-core-based SpMM implementations, while achieving only slightly lower performance on matrices that do not exhibit TCU-Synergy.


==> sections/discussion.tex <==

\label{sec:ongoing}
The experimental evaluatin of cuTESpMM shows very significant speedup over Nvidia's cuSparse Blocked-ELL library. However, the improvement in performance over the standard cuSparse CSR library is dependent on the 2D clustering density within the non-empty bricks. In order to increase the practical utility and impact of cuTESpMM, we are currently pursuing two research directions:

\paragraph{Matrix Reordering}
We are evaluating the impact of row/column reordering of sparse matrices on the non-zero density within 2D blocks in portions of the index space of the sparse matrix, so that more effective use may be made of the TCUs. In addition to evaluating existing reordering schemes like Reverse Cuthill-McKee aimed, we are also new developing reordering strategies 

\paragraph{Model-Driven Selection}

We are also working on an analytical/machine learning model to extract the features of the matrix and use them to predict when performance using cuTESpMM is expected to be higher than using cuSparse CSR.
% -Talk about the ongoing work "on reordering that can increase the number of matrices where the kernel is expected to outperform CSR"


==> sections/experiment-old.tex <==
\subsection{Hardware Setting and Datasets}
\label{sec:setting}

\begin{figure*}[]
\centering
\includegraphics[width=0.99\linewidth]{figs/perf-ell.pdf}
\caption{Performance Comparison: cuTeSpMM vs. cuSparse Blocked-ELL}
\label{fig:perf-ell}
\end{figure*}

Our experiments were performed on two  Nvidia graphics processing units (GPUs): an Ampere-A100 with 80GB memory, and an RTX-A6000 with 48GB memory. These GPUs were hosted on machines running the RockyLinux8 operating system, using CUDA 11.8, with 150GB of RAM.
%\begin{figure}[h!]
%\centering
%\includegraphics[width=0.85\linewidth]{figs/datasets.png}
%\caption{Datasets summary}
%\label{fig:dataset}
%\end{figure}

We utilized a diverse set of 356 matrices from the SuiteSparse collection\cite{davis2011university}. Since we are primarily interested in using GPUs for large matrices, only matrices with more than 50,000 rows/columns were selected. Some matrices were too large to fit the sparse and dense matrices for SpMM into GPU memory and were excluded. The median values for the number of non-zero entries (NNZ) and rows were 200,000 and 2 million respectively. The median density was 6.10E-05. Size statistics on the selected matrices are presented in Table~\ref{tab:my-table} (full details on the list of matrices will be provided with the Artifact Description).

\begin{table}[]
\caption{Distribution of sparse matrix sizes}
\todo[inline]{\large Create a 2D table with M and NNZ bins?}
\begin{tabular}{|l|l|l|l|}
\hline
$\#Rows$     & $\#Matrices$ & $\#NNZ$    & $\#Matrices$ \\ \hline
50K-100K & 125                & 30K-1M         & 136                \\ \hline
100K-200K          & 82                 & 1M-5M   & 120                \\ \hline
200K-300K          & 42                 & 5M-10M   & 39                 \\ \hline
300K-400K          & 24                 & 10M-20M & 40                 \\ \hline
400K-500K          & 17                 & \textgreater{}20M &   21                 \\ \hline
500K-1M            & 40                 &      &                   \\ \hline
\textgreater{}1M   & 26                 &      &                  \\ \hline
\end{tabular}

\label{tab:my-table}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% Please adrd the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


\subsection{Comparison with cuSparse Blocked-ELL}
\label{sec:results}


Fig.~\ref{fig:perf-ell} presents performance data for cuTeSpMM in comparison with Nvidia cuSParse Blocked-ELL SpMM, for the two GPUs, for three dense-matrix widths: 16, 32, 64. For cuSParse Blocked-ELL SpMM, we varied the block size for Blocked-ELL representation over a number of values and found that a block size of 32 was consistently the best and so used that block size for all experiments. Each of the six charts plots achieved performance in GFLOPs by Blocked-ELL on the X-axis and cuTeSpMM performance on the Y-axis. Thus, all points above the 45 degree diagonal line represent matrices where cuTeSpMM achieved higher performance. It may be seen that except for a handful of matrices out of the 356 test matrices, cuTeSpMM achieves higher performance. Performance on the A-100 was higher than on th RTX-6000 for both cuTeSpMM and Blocked-ELL. As the dense matrix width is increased from 16 to 32 to 64, the achieved performance for both cuTeSpMM and Blocked-ELL increase.

\begin{figure*}[]
\centering
\includegraphics[width=0.99\linewidth]{figs/perf-csr.pdf}
\caption{Performance Comparison: cuTeSpMM vs. cusparse CSR}
\label{fig:perf-csr}
\end{figure*}
\subsection{Comparison with cuSparse-CSR}
Fig.~\ref{fig:perf-csr} presents performance data for cuTeSpMM in comparison with Nvidia cuSParse CSR, for the two GPUs, and the three dense-matrix widths. In contrast to the comparison with Blocked-ELL, cuTE is only faster than cuSparse-CSR forroughly half the matrices. However, it may be seen that the highest achieved performance is considerably higher with cuTeSpMM. For example, on the A-100 GPU the highest achieved performance by cuSparse-CSR on any matrix is around 300 GFLOPs for dense-matrix width W=16, around 600 GFLOPs for W=32, and around 1000 GFLOPs for W=64. For cuTeSpMM, the corresponding performance numbers for W=16/32/64 are around 2400/2500/5500 GFLOPs.

\begin{table*}[!t]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|} 
\hline
\multicolumn{1}{|l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{A100} & \multicolumn{1}{l}{} &      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{A6000} & \multicolumn{1}{l}{} &       \\ 
\hline
Feature Size          & 16                   & 32                       & 64                   & All  & Feature Size         & 16                   & 32                        & 64                   & All   \\ 
\hline
CSR                   & 1.34                 & 1.07                     & 1.04                 & 1.14 & CSR                  & 0.86                 & 0.75                      & 0.89                 & 0.83  \\ 
\hline
BELL                  & 6.87                 & 4.84                     & 5.10                 & 5.54 & BELL                 & 9.49                 & 7.68                      & 6.23                 & 7.69  \\
\hline
\end{tabular}
\label{tab:geomean-all}
\caption{Geometric mean speedup over all test matrices: cuTESpMM vs. cuSparse CSR and cuSparse Blocked-ELL }
\end{table*}

In Table ~\ref{tab:geomean-all}, we summarize the performance measurements by reporting the geometric mean of achieved speedup of cuTESpMM over cuSparse CSR and Blocked-ELL, across all 356 test matrices, for the three dense-matrix widths, on both target platforms. It may be seen that the performance improvements over Blocke-ELL are very significant on both machines, with the speedups being higher on the A6000 system. On the A-100, speedup is obtained overall for all widths of the dense matrix, while on the A6000 the geometric mean speedup is less than one. A reason for the different trends across the A100 and A6000 is explained by the relative performance of tensor cores versus CUDA cores on the two systems: the peak tensor core performance is 156 TFLOPs on the A100 and 77.4 TFLOPs on the A6000, whereas the peak scalar CUDA-core performance is only 19.5 TFLOPs for the A100, while it is 38.7 TFLOPs for the A6000. 

%\begin{figure*}[]
%\centering
%\includegraphics[width=0.99\linewidth]{figs/perf-ell-.1.pdf}
%\caption{cuTeSpMM vs. cuSparse Blocked-ELL Performance, "average brick density"  $>= %\0.1$}
%\label{fig:perf-ell1}
%\end{figure*}

A key attribute of sparse matrices that has a direct impact on achieved performance with cuTeSpMM is the non-zero density within non-empty $16 \times 4$ 2D regions in the full 2D index space of the sparse matrix. This is because explicit zero-filling must be used for the remaining elements in order to use the tensor core's matrix-matrix multiplication engine. Since the tensor core's peak performance of Nvidia GPUs for TF32 tends to be about an order of magnitude higher than the performance using the standard scalar ``CUDA cores'', we also assessed the relative performance of cuTeSpMM over cuSparse Blocked-ELL over a subset of the test matrices with non-zero brick density of at least 10\% (this was 133 matrices out of 356). These performance results are presented in Fig.~\ref{fig:perf-ell1}. It may be seen that the fraction of matrices achieving higher performance than cuSparse CSR is much higher. The geometric means of speedup for the subset of matrices with brick nnzero density greater than 10\% is reported in Table ~\ref{tab:geomean-1}. For such matrices, the speedup over cuSparse CSR is always greater than one. The speedup over Blocked-ELL is lower for these matrices because blocked-ELL performance is relatively higher for these denser matrices.

\begin{figure*}[]
\centering
\includegraphics[width=0.99\linewidth]{figs/perf-csr-.1.pdf}
\caption{cuTeSpMM v.s. cusparse CSR Performance Plots, "average brick density" $>= 0.1$}
\label{fig:perf-csr1}
\end{figure*}

% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{figs/perf-n32-a100.pdf}
%         \caption{feature size = 32}
%     \end{subfigure}%
%     \hfill

%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{figs/perf-n64-a100.pdf}
%         \caption{feature size = 64}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{figs/perf-n128-a100.pdf}
%         \caption{feature size = 128}
%     \end{subfigure}
    
%     \caption{GPU=a100}
% \end{figure*}

% \begin{figure*}[t!]
%     \centering
%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{figs/perf-n32-a6000.pdf}
%         \caption{feature size = 32}
%     \end{subfigure}%
%     \hfill

%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{figs/perf-n64-a6000.pdf}
%         \caption{feature size = 64}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}[t]{\textwidth}
%         \centering
%         \includegraphics[width=.9\textwidth]{figs/perf-n128-a6000.pdf}
%         \caption{feature size = 128}
%     \end{subfigure}
    
%     \caption{GPU=a6000}
% \end{figure*}

\begin{table*}[!t]
\centering
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|} 
\hline
\multicolumn{1}{|l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{A100} & \multicolumn{1}{l}{} &      & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{A6000} & \multicolumn{1}{l}{} &       \\ 
\hline
Feature Size          & 16                   & 32                       & 64                   & All  & Feature Size         & 16                   & 32                        & 64                   & All   \\ 
\hline
CSR                   & 2.18                 & 1.67                     & 1.62                 & 1.80 & CSR                  & 1.41                 & 1.13                      & 1.06                 & 1.19  \\ 
\hline
BELL                  & 4.48                 & 3.10                     & 3.30                 & 3.58 & BELL                 & 6.00                 & 4.80                      & 3.90                 & 4.83  \\
\hline
\end{tabular}
\caption{Geometric mean speedup over subset of test matrices with "average brick density"  $>= 0.1$: cuTESpMM vs. cuSparse CSR and cuSparse Blocked-ELL}
\label{tab:geomean-1}
\end{table*}

\subsection{Comparision with TC-GNN SpMM}
\label{sec:tc-gnn}
Besides Nvidia's cuSparse Blocked-ELL SpMM, the only other effort to use tensor cores for SpMM (to our knowledge) is TC-GNN\cite{wang2021tc}. TC-GNN implements Graph Neural Networks (GNN), where SpMM is a dominant computational component. However, the SpMM implementation within TC-GNN is highly integrated with Pytorch and no API is available for directly executing the internal SpMM implementation to perform a direct comparison with  cuTeSpMM. Although we were not able perform a direct experimental comparison with TC-GNN's SpMM implementtaion,  we report the speedup achieved by cuTeSpMM over cuSparse Blocked-ELL on five specific sparse matrices reported by Wang et al. \cite{wang2021tc}, using a similar GPU (they used an Nvidia RTX3090, which is quite similar in overall performance to the Nvidia RTX A6000 we use as one of two GPUs for our experimets). Table~\ref{tab:geomean-1} shows that the achieved speedup of cuTeSpMM over cuSparse Blocked-ELL is very much higher than the speedup reported by Wang et al. \cite{wang2021tc}.

\begin{table}[]
\caption{Performance improvement (speedup) of cuTeSpMM  and TC-GNN over Blocked-ELL}
\begin{tabular}{|l|l|l|}
\hline
$Matrix$     & cuTeSpMM & TC-GNN \cite{wang2021tc}   \\ \hline
amazon0505   & 27.92 & 4.55 \\ \hline
amazon0601   & 26.28 & 3.5 \\ \hline
$com-Amazon$ & 65.9 & 4.25 \\ \hline
artist & 24.4 & 2.99 \\ \hline
$soc-BlogCatalog$ &19.79 & 2.71 \\ \hline
\end{tabular}

\label{tab:speedup tc-gnn}
\end{table}

==> sections/modeling.tex <==
CuTeSpMM is not uniformly faster than CSR. The choice between the two algorithms depends on the distribution of non-zero elements in the sparse matrix. Once we have a suitable representation of the sparse matrix, we can utilize a machine learning model to predict the optimal algorithm. Machine learning models are adept at capturing low-level features that can translate into high-level features. However, it is challenging to obtain an accurate representation of the sparse matrix while preserving sufficient information.

One straightforward approach is to pass the sparse matrix as a dense matrix, retaining all the zero values. This would provide the model with all the features of the sparse matrix. However, this method is not feasible due to the excessive memory required for the dense feature map.

Another option is to encode the sparse matrix using compression methods like CSR and design a language model accordingly. However, this approach also has limitations, as even a compressed sparse matrix may contain millions of elements, exceeding the capabilities of standard language models.

Zhao proposed a CNN network for the design of a sparse algorithm classification model, specifically for predicting the optimal sparse algorithm/data format (CSR, COO, DIA, ELL) for SpMV operations. Zhao employed image down-sampling on the sparse matrix to generate a 128x128 feature map. Each block in the original matrix corresponded to a value in the feature map, representing the density of that block. This feature map was then used for classification within the CNN network.

While Zhao's model utilized a similar CNN architecture, we employ a different representation of the sparse matrix. This is because downsampling the matrix to a small size, such as 128x128 as in Zhao's approach, does not provide sufficient information about the individual bricks within each block. Ideally, we aim to capture the density of each brick inside a block, which requires a distinct representation.

Constructing a feature map where each value represents the density of a brick is indeed possible. However, it would require ${(M*N)/(brick_m*brick_n)}$ memory, making it impractical for large matrices. Therefore, we need to find alternative approaches to effectively represent the sparse matrix and its features.\par


In our modeling design, we represent the sparse matrix using 5 feature vectors. Each vector corresponds to a row panel and contains values representing specific features. The 5 features we are interested in for each row panel are as follows:

1)Density of the row panel: This feature represents the density of non-zero elements in the row panel.

2)Number of active bricks in the row panel: This feature indicates the count of active bricks (bricks with non-zero elements) in the row panel.

3)Average density of each brick: This feature calculates the average density of the individual bricks within the row panel.

4)Average number of active bricks in a brick column of the row panel: This feature computes the average number of active bricks in each column of the row panel.

5)Standard deviation of the number of active bricks in a brick column: This feature measures the variability or spread in the number of active bricks across the columns of the row panel.\par
The five feature vectors are combined to create a 5-channel feature map, which is then inputted into our custom-designed CNN model for prediction. Please refer to Figure ??\textcolor{red}{Todo Draw the CNN architecure} for a visual representation of our model's architecture.

==> sections/parameters.tex <==
\textcolor{red}{In our kernel design, two parameters, ${TM, TK}$  represent the dimension sizes along 
 $(M, k)$ of a block inside a row panel. The TK size is fixed to 16 in our kernel design. The TK size does not directly affect data movement and the amount of FMA computations which are the two crucial factors regarding performance, since each thread block is streaming along the entire K dimension. However, it still impacts the kernel in various ways. In line XX in our kernel design algorithm, we are traverse all the ${\frac{TK}{brick_k}}$ brick columns inside a block. This for loop is fully unrolled as ${TK}$ and ${brick_k}$ are constants. Inside the for loop, the prefix scanning operations we employ to decode the non-zero distribution pattern are entirely independent. A large TK value benefits ILP (Instruction-Level Parallelism), potentially improving the performance.  However, a larger TK value also increases shared memory usage. The total shared memory usage is determined by ${2 \times TM \times TK + MetaDatasize + 2\time TK * N}$(where the factor of 2 accounts for double buffering on both ${SM\_A}$ and ${SM\_B}$ buffers to hide the data movement latency from global memory). Shared memory is a very constrained resource on GPUs, and increased shared memory usage can lead to a drop in occupancy, potentially degrading parallelism. In practice, quantifying the benefits of an increased ILP level is challenging. From a programmer's perspective, even ILP level isn't entirely within our control, as it's ultimately determined by the compiler. Therefore, we determined the ${TK}$ size by running numerous matrices with various ${TK}$ sizes, ultimately choosing a size of 16.}
 ${TM}$ is the height of a row panel size. From data movement prospective, a large ${TM}$ may increase the data reuse level of the ${B}$ matrix. In line xx of our cuTeSpMM algorithm, we use the colptr to traverse the active bricks, all the active bricks in a brick column require same elements from the B matrix. For a dense matrix, the number of active bricks in a brick column is ${\frac{TM}{brick_m}}$.   

==> sections/plots.tex <==
% ########################################  BOX CHARTS ##########################################




% \begin{figure*}[htbp]
%   \centering
%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{figs/plots/boxChart_TCGNN-BELL-bestCuda/a100_boxCharts_all_F_category_High.png}
%     % \caption{F=512}
%     % \label{fig:f512}
%   \end{subfigure}
  
%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{figs/plots/boxChart_TCGNN-BELL-bestCuda/a100_boxCharts_all_F_category_Medium.png}
%     % \caption{F=128}
%     % \label{fig:f128}
%   \end{subfigure}
  
%   \begin{subfigure}[b]{0.7\textwidth}
%     \includegraphics[width=\textwidth]{figs/plots/boxChart_TCGNN-BELL-bestCuda/a100_boxCharts_all_F_category_Low.png}
%     % \caption{F=32}
%     % \label{fig:f32}
%   \end{subfigure}
  
%   \caption{Comparing TCGNN, best-CUDA, and cuELLBlk on different synergy groups}
%   % \label{fig:boxplots}
% \end{figure*}

% ########################################  HISTOGRAMS ##########################################

%%%%%%%%%%%%%%%%%%%% cuteSpMM speedup over Best of TCU
% \begin{figure*}[htbp]
%   \centering
%   \begin{subfigure}[b]{\columnwidth}
%     \includegraphics[width=\textwidth]{figs/plots/hists_cuteSpMM-speedup/a100_TCU_speedup_plot_category_High.png}
%     % \caption{F=512}
%     % \label{fig:f512}
%   \end{subfigure}
  
%   \begin{subfigure}[b]{\columnwidth}
%     \includegraphics[width=\textwidth]{figs/plots/hists_cuteSpMM-speedup/a100_TCU_speedup_plot_category_Medium.png}
%     % \caption{F=128}
%     % \label{fig:f128}
%   \end{subfigure}

%   \begin{subfigure}[b]{\columnwidth}
%     \includegraphics[width=\textwidth]{figs/plots/hists_cuteSpMM-speedup/a100_TCU_speedup_plot_category_Low.png}
%     % \caption{F=32}
%     % \label{fig:f32}
%   \end{subfigure}
%   \caption{cuteSpMM speedup over Best of TCU for different feature sizes}
%   \label{fig:boxplots}
% \end{figure*}

%%%%%%%%%%%%%%%%%%%% cuteSpMM speedup over Best of CUDA
% \begin{figure}[htbp] 
%   \centering
%   \begin{subfigure}[b]{\columnwidth}
%     \includegraphics[width=\textwidth]{figs/plots/hists_cuteSpMM-speedup/a100_CUDA_speedup_plot_category_High.png}
%     % \caption{F=512}
%     % \label{fig:f512}
%   \end{subfigure}
  
%   \begin{subfigure}[b]{\columnwidth}
%     \includegraphics[width=\textwidth]{figs/plots/hists_cuteSpMM-speedup/a100_CUDA_speedup_plot_category_Medium.png}
%     % \caption{F=128}
%     % \label{fig:f128}
%   \end{subfigure}

%   \begin{subfigure}[b]{\columnwidth}
%     \includegraphics[width=\textwidth]{figs/plots/hists_cuteSpMM-speedup/a100_CUDA_speedup_plot_category_Low.png}
%     % \caption{F=32}
%     % \label{fig:f32}
%   \end{subfigure}
%   \caption{cuteSpMM speedup over Best of CUDA for different feature sizes}
%   \label{fig:boxplots}
% \end{figure}

\clearpage
%   % @omid: TODO: 
%   %  right should be a100 left H100
%   %  remove the y-axis ticks for H100  

% @omid DONE: change this to speedup over all


%%%%%%%%%%%%%%%%%%%%%%%%%%%% TABLES
% yes 


\begin{table*}[ht]
\footnotesize % Smaller font size
\centering
\setlength{\tabcolsep}{4pt} % Reduce column padding
\begin{tabular}{l|cccc|cccc|cccc}
\textbf{Matrix} & \multicolumn{4}{c|}{n=32} & \multicolumn{4}{c|}{n=64} & \multicolumn{4}{c}{n=128} \\
\cline{2-5} \cline{6-9} \cline{10-13}
 & \rotatebox{90}{cuTeSpMM} & \rotatebox{90}{bSpMM} & \rotatebox{90}{TC-GNN} & \rotatebox{90}{Best-SC} & \rotatebox{90}{cuTeSpMM} & \rotatebox{90}{bSpMM} & \rotatebox{90}{TC-GNN} & \rotatebox{90}{Best-SC} & \rotatebox{90}{cuTeSpMM} & \rotatebox{90}{bSpMM} & \rotatebox{90}{TC-GNN} & \rotatebox{90}{Best-SC} \\
\hline
amazon0505 & 857 & - & 122 & 811 & 1024 & - & 202 & 746 & 1077 & - & 271 & 940 \\
amazon0601 & 815 & 15 & 161 & 991 & 988 & 24 & 274 & 669 & 1049 & 39 & 383 & 899 \\
artist & 510 & 9 & 73 & 626 & 655 & 15 & 135 & 864 & 782 & 27 & 202 & 1361 \\
citeseer & 56 & 7 & 13 & 41 & 105 & 15 & 26 & 93 & 176 & 28 & 47 & 152 \\
com-amazon & 455 & 3 & 98 & 467 & 587 & 5 & 170 & 447 & 657 & 8 & 249 & 616 \\
cora & 59 & 11 & 10 & 45 & 113 & 21 & 20 & 81 & 205 & 36 & 37 & 150 \\
DD & 821 & 29 & 177 & 767 & 1034 & 39 & 302 & 560 & 1150 & 75 & 426 & 925 \\
OVCAR-8H & 497 & 67 & 117 & 396 & 611 & 123 & 196 & 454 & 674 & 228 & 275 & 508 \\
ppi & 587 & 55 & 107 & 720 & 717 & 84 & 198 & 708 & 929 & 158 & 297 & 1235 \\
PROTEINS\_full & 457 & 64 & 126 & 515 & 690 & 99 & 220 & 445 & 788 & 188 & 330 & 633 \\
pubmed & 269 & 4 & 43 & 233 & 359 & 5 & 79 & 325 & 502 & 11 & 131 & 581 \\
soc-BlogCatalog & 863 & 17 & 69 & 638 & 1079 & 24 & 126 & 989 & 1374 & 47 & 191 & 1644 \\
Yeast & 507 & 80 & 125 & 401 & 627 & 159 & 209 & 454 & 695 & 289 & 295 & 507 \\
YeastH & 499 & -done & 118 & 393 & 615 & - & 198 & 457 & 667 & - & 276 & 495 \\
\hline
\end{tabular}
\caption{Comparing the performance(GFLOPs) of cuTeSpMM, TC-GNN, bSpMM, and Best-Scalar for matrices tested in \cite{wang2023tc}}%\PS{Why are there zero entries?} \PS{Names need to be made consistent in Table}}
\label{table:TCGNN}
\end{table*}








==> sections/related.tex <==

% \ASR{Why are we talking about sparse tensor cores? we are not using it. Instead we can add something like the following at the end of (2.1). "While Nvidia Ampere Architecture GPU has added support for sparse multiplication using tensor cores, it only supports 2:4 sparsity pattern (in a contiguous block of 4 elements, two should be zero), and hence is not compatible with generic sparse matrices used in SpMM"}

